Optimal communication and control strategies in a multi-agent MDP problem

The problem of controlling multi-agent systems under different models of information sharing among agents has received significant attention in the recent literature. In this paper, we consider a setup where rather than committing to a fixed information sharing protocol (e.g. periodic sharing or no sharing etc), agents can dynamically decide at each time step whether to share information with each other and incur the resulting communication cost. This setup requires a joint design of agents' communication and control strategies in order to optimize the trade-off between communication costs and control objective. We first show that agents can ignore a big part of their private information without compromising the system performance. We then provide a common information approach based solution for the strategy optimization problem. This approach relies on constructing a fictitious POMDP whose solution (obtained via a dynamic program) characterizes the optimal strategies for the agents. We also show that our solution can be easily modified to incorporate constraints on when and how frequently agents can communicate.

==> AN_AppC.tex <==
%%%Dhruva: Use this file for editing  Appendix C%%%


\section{Proof of Lemma \ref{LEM:UPDATE}}\label{proof:Coord}
Recall that at the beginning of time $t$, the common information is given by $C_{t}:=(Z_{1:t-1},M^{1,2}_{1:t-1})$ (see \eqref{commoninfo}).
At the end of time $t$, i.e. after the communication decisions are made at time $t$, the common information is given by $C_{t^+}:=(Z_{1:t},M^{1,2}_{1:t})$ (see \eqref{commoninfoplus}). Let $c_{t} := (z_{1:t-1},m_{1:t-1}^{1,2})$ and $c_{t^+} := (z_{1:t},m_{1:t}^{1,2})$ be realizations of $C_t$ and $C_{t^+}$ respectively. Let $\gamma_{1:t},\lambda_{1:t-1}$ be the realizations of the coordinator's prescriptions $\Gamma_{1:t},\Lambda_{1:t-1}$ up to time $t$. Let us assume that the realizations $c_{t^+},\gamma_{1:t},\lambda_{1:t-1}$ have non-zero probability. Then the corresponding realizations $\pi_t$ and $\pi_{t^+}$ of the coordinator's beliefs $\Pi_t$ and $\Pi_{t^+}$ are given by:
\begin{align}
\pi_{t}(x_t)&=\prob(X_t=x_t|C_t=(z_{1:t-1},m^{1,2}_{1:t-1}),\Gamma_{1:t-1}=\gamma_{1:t-1},\Lambda_{1:t-1}=\lambda_{1:t-1})\label{updatelem3:1}\\
    \pi_{t^+}(x_{t^+})&=\prob(X_{t}=x_{t}|C_{t^+}=(z_{1:t},m^{1,2}_{1:t}),\Gamma_{1:t}=\gamma_{1:t},\Lambda_{1:t-1}=\lambda_{1:t-1}).\label{updatelem3:2}
\end{align}
For $i=1,2$, let $\pi_t^i$ (resp. $\pi_{t^+}^i$) be the realization of the coordinator's belief $\Pi_t^i$ (resp. $\Pi_{t^+}^i$) on $X_t^i$. From Lemma \ref{LEM:INDEPEN}, we have
\begin{align}
\label{factor1}\pi_t(x_t) &= \pi_t^1(x_t^1)\pi_t^2(x_t^2) ~~\forall x_t\\
\label{factor2}\pi_{t^+}(x_t) &= \pi_{t^+}^1(x_t^1)\pi_{t^+}^2(x_t^2) ~~\forall x_t.
\end{align}


There are two possible cases: (i) $z_t = (\tilde{x}_t^{1},\tilde{x}_t^{2})$ for some $(\tilde{x}_t^{1},\tilde{x}_t^{2}) \in \mathcal{X}^1\times \mathcal{X}^2$ or (ii) $z_t = \phi$. Let us analyze these two cases separately.

\textbf{Case I:} When $z_t = (\tilde{x}_t^{1},\tilde{x}_t^{2})$ for some $(\tilde{x}_t^{1},\tilde{x}_t^{2}) \in \mathcal{X}^1\times \mathcal{X}^2$, at least one of the agents must have decided communicated at time $t$. As described in \eqref{zt}, the variable $Z_t = X_t$ when communication occurs. Thus, we have
\begin{align}
    \pi_{t^+}(x_t)&=\prob(X_t=x_{t}|z_{1:t},m^{1,2}_{1:t},\gamma_{1:t},\lambda_{1:t-1})\notag\\
    &=\mathds{1}_{(\tilde{x}^{1}_{t}=x^1_t)}\mathds{1}_{(\tilde{x}^{2}_{t}=x^2_t)}, \label{updatelem3:3}
\end{align}
where $x_t = (x^1,x^2)$. Further, we have
\begin{align}
\label{indupdate1}\pi_{t^+}^i(x_t^i) = \mathds{1}_{(\tilde{x}^{i}_{t}=x^i_t)}, ~~i = 1,2.
\end{align}



\textbf{Case II:} When ${z}_t=\phi$, it implies that there was no communication at time $t$ and hence, ${m}^{1,2}_t=(0,0)$ (see \eqref{zt}). Using the Bayes' rule, we have
\begin{align}
    \pi_{t^+}(x_t)&=P(X_t=x_{t}|z_{1:t},m^{1,2}_{1:t},\gamma_{1:t},\lambda_{1:t-1})\notag\\
    &=\frac{P(X_t=x_{t},Z_t=\phi,M^{1,2}_t=(0,0)|z_{1:t-1},m^{1,2}_{1:t-1},\gamma_{1:t},\lambda_{1:t-1})}{P(Z_t=\phi,M^{1,2}_t=(0,0)|z_{1:t-1},m^{1,2}_{1:t-1},\gamma_{1:t},\lambda_{1:t-1})}\notag\\
    &=\frac{P(Z_t=\phi|x_{t},c_t,\gamma_{1:t},\lambda_{1:t-1},M^{1,2}_t=(0,0))P(M^{1,2}_t=(0,0)|x_t,c_t,\gamma_{1:t},\lambda_{1:t-1}) P(X_t=x_{t}|c_t,\gamma_{1:t},\lambda_{1:t-1})   }{\sum_{\hat{x}_t}P(Z_t=\phi|\hat{x}_{t},c_t,\gamma_{1:t},\lambda_{1:t-1},M^{1,2}_t=(0,0))P(M^{1,2}_t=(0,0)|\hat{x}_t,c_t,\gamma_{1:t},\lambda_{1:t-1}) P(X_t=\hat{x}_{t}|c_t,\gamma_{1:t},\lambda_{1:t-1})   }\notag\\
    &\stackrel{a}{=}\frac{P(M^{1,2}_t=(0,0)|x_t,c_t,\gamma_{1:t},\lambda_{1:t-1}) P(X_t=x_{t}|c_t,\gamma_{1:t},\lambda_{1:t-1})  }{\sum_{\hat{x}_t} P(M^{1,2}_t=(0,0)|\hat{x}_t,c_t,\gamma_{1:t},\lambda_{1:t-1})P(X_t=\hat{x}_{t}|c_t,\gamma_{1:t},\lambda_{1:t-1}) }\notag\\
    &\stackrel{b}{=}\frac{P(M^{1,2}_t=(0,0)|x_t,c_t,\gamma_{1:t},\lambda_{1:t-1}) P(X_t=x_{t}|c_t,\gamma_{1:t-1},\lambda_{1:t-1})  }{\sum_{\hat{x}_t} P(M^{1,2}_t=(0,0)|\hat{x}_t,c_t,\gamma_{1:t},\lambda_{1:t-1})P(X_t=\hat{x}_{t}|c_t,\gamma_{1:t-1},\lambda_{1:t-1}) }\notag\\
    &\stackrel{c}{=}\frac{\mathds{1}_{(\gamma^1_t(x^1_t)=0)}\mathds{1}_{(\gamma^2_t(x^2_t)=0)}P(X_t=x_{t}|c_t,\gamma_{1:t-1},\lambda_{1:t-1}) }{\sum_{\hat{x}_t}\mathds{1}_{(\gamma^1_t(\hat{x}^1_t)=0)}\mathds{1}_{(\gamma^2_t(\hat{x}^2_t)=0)}P(X_t=\hat{x}_{t}|c_t,\gamma_{1:t-1},\lambda_{1:t-1})}\notag\\ 
    &=\frac{\mathds{1}_{(\gamma^1_t(x^1_t)=0)}\mathds{1}_{(\gamma^2_t(x^2_t)=0)}\pi_t(x_t)}{\sum_{\hat{x}_t}\mathds{1}_{(\gamma^1_t(\hat{x}^1_t)=0)}\mathds{1}_{(\gamma^2_t(\hat{x}^2_t)=0)}\pi_t(\hat{x}_t)}\\
    &\stackrel{d}{=}\frac{\mathds{1}_{(\gamma^1_t(x^1_t)=0)}\mathds{1}_{(\gamma^2_t(x^2_t)=0)}\pi_t^1(x_t^1)\pi_t^2(x_t^2)}{\sum_{\hat{x}_t}\mathds{1}_{(\gamma^1_t(\hat{x}^1_t)=0)}\mathds{1}_{(\gamma^2_t(\hat{x}^2_t)=0)}\pi_t^1(\hat{x}_t^1)\pi_t^2(\hat{x}_t^2)} \\
    &= \left(\frac{\mathds{1}_{(\gamma^1_t(x^1_t)=0)}\pi_t^1(x_t^1)}{\sum_{\hat{x}^1_t}\mathds{1}_{(\gamma^1_t(\hat{x}^1_t)=0)}\pi_t^1(\hat{x}_t^1)}\right) \times \left(\frac{\mathds{1}_{(\gamma^2_t(x^2_t)=0)}\pi_t^2(x_t^2)}{\sum_{\hat{x}^2_t}\mathds{1}_{(\gamma^2_t(\hat{x}^2_t)=0)}\pi_t^2(\hat{x}_t^2)}\right).\label{updatelem3:4}
\end{align}
In the display above, equality $(a)$ follows from the fact that $Z_t = \phi$ if and only if $M^{1,2}_t = (0,0)$ (see \eqref{zt}). In equation $(b)$, we drop $\gamma_t$ from the term $ P(X_t=x_{t}|c_t,\gamma_{1:t},\lambda_{1:t-1})$ because $\gamma_t$ is a function of the rest of them terms in the conditioning given the coordinator's strategy. Equation $(c)$ is a direct consequence of the selection rule in \eqref{commact1}. Equation $(d)$ follows from the result in \eqref{factor1}. Further, using the result in \eqref{updatelem3:4}, we have
\begin{align}
\label{indupdate2}\pi_{t^+}^i(x_t^i) = \frac{\mathds{1}_{(\gamma^i_t(x^i_t)=0)}\pi_t^i(x_t^i)}{\sum_{\hat{x}^i_t}\mathds{1}_{(\gamma^i_t(\hat{x}^i_t)=0)}\pi_t^i(\hat{x}_t^i)},~~i = 1,2. 
\end{align}
From the results in \eqref{indupdate1} and \eqref{indupdate2}, we can update the coordinator's beliefs $\pi_{t^+}^i$ ($i=1,2$) using $\pi_t^i,\gamma_t^i$ and $z_t$ as:
\begin{equation}
  \pi^i_{t^+}(x_t^i)=\begin{cases}
    \frac{\mathds{1}_{(\gamma^i_t(x^i_t)=0)}\pi_t^i(x_t^i)}{\sum_{\hat{x}^i_t}\mathds{1}_{(\gamma^i_t(\hat{x}^i_t)=0)}\pi_t^i(\hat{x}_t^i)}, & \text{if $z_t=\phi$}.\\
    \mathds{1}_{(x^i_t=\Tilde{x}^i_t)}, & \text{if $z_t =  (\tilde{x}_t^{1},\tilde{x}_t^{2})$}.
  \end{cases}\label{updatelem3:11}
\end{equation}
We denote the update rule described above with $\eta^i_t$, i.e.
\begin{align}
\pi_{t^+}^i = \eta_t^i(\pi_t^i,\gamma_t^i,z_t).
\end{align}



Let $c_{t+1} := (z_{1:t},m_{1:t}^{1,2})$ be a realization of $C_{t+1}$. Let $\gamma_{1:t},\lambda_{1:t}$ be the realizations of the coordinator's prescriptions $\Gamma_{1:t},\Lambda_{1:t}$ up to time $t$. Let us assume that the realizations $c_{t+1},\gamma_{1:t},\lambda_{1:t}$ have non-zero probability. Then the corresponding realizations $\pi_{t+1}$ of the coordinator's beliefs $\Pi_{t+1}$ is given by:
\begin{align}
\pi_{t+1}(x_{t+1})&=\prob(X_{t+1}=x_{t+1}|C_{t+1}=(z_{1:t},m^{1,2}_{1:t}),\Gamma_{1:t}=\gamma_{1:t},\Lambda_{1:t}=\lambda_{1:t})
\end{align}
For $i=1,2$, let $\pi_{t+1}^i$ be the realization of the coordinator's belief $\Pi_{t+1}^i$ on $X_t^i$. From Lemma \ref{LEM:INDEPEN}, we have
\begin{align}
\label{factor3}\pi_{t+1}(x_{t+1}) &= \pi_{t+1}^1(x_{t+1}^1)\pi_{t+1}^2(x_{t+1}^2) ~~\forall x_{t+1}.
\end{align}

Using the law of total probability, we have

\begin{align}
    &\pi_{t+1}(x_{t+1})\\
    &=\prob(X_{t+1} =x_{t+1}|z_{1:t},m^{1,2}_{1:t},\gamma_{1:t},\lambda_{1:t})\\
    &= \sum_{x_t}\sum_{u_t}\prob(X_{t+1} = x_{t+1}|x_t,u_t,z_{1:t},m^{1,2}_{1:t},\gamma_{1:t},\lambda_{1:t})\prob(U_t = u_t|x_t,z_{1:t},m^{1,2}_{1:t},\gamma_{1:t},\lambda_{1:t})\prob(X_t  =x_{t}|z_{1:t},m^{1,2}_{1:t},\gamma_{1:t},\lambda_{1:t})\\
    &\stackrel{a}{=} \sum_{x_t}\sum_{u_t}\prob(X_{t+1} = x_{t+1}|x_t,u_t,z_{1:t},m^{1,2}_{1:t},\gamma_{1:t},\lambda_{1:t})\prob(U_t = u_t|x_t,z_{1:t},m^{1,2}_{1:t},\gamma_{1:t},\lambda_{1:t})\prob(X_t = x_{t}|z_{1:t},m^{1,2}_{1:t},\gamma_{1:t},\lambda_{1:t-1})\\
    &\stackrel{b}{=} \sum_{x_t}\sum_{u_t}\prob(X_{t+1} = x_{t+1}|x_t,u_t,z_{1:t},m^{1,2}_{1:t},\gamma_{1:t},\lambda_{1:t})\mathds{1}_{(u_t=\lambda_t(x_t))}\pi_{t^+}(x_t)\\
    &\stackrel{c}{=} \sum_{x_t}\sum_{u_t}\prob(X_{t+1} = x_{t+1}|x_t,u_t)\mathds{1}_{(u_t=\lambda_t(x_t))}\pi_{t^+}(x_t)\\
    &\stackrel{d}{=} \sum_{x_t}\sum_{u_t}\prob(X^1_{t+1}=x^1_{t+1}|x^1_t,u^1_t)\prob(X^2_{t+1}=x^2_{t+1}|x^2_t,u^2_t)\mathds{1}_{(u^1_t=\lambda^1_t(x^1_t))}\mathds{1}_{(u^2_t=\lambda^2_t(x^2_t))}\pi^1_{t^+}(x^1_{t})\pi^2_{t^+}(x^2_{t})\\
    &= \left(\sum_{x_t^1}\sum_{u_t^1}\prob(X^1_{t+1}=x^1_{t+1}|x^1_t,u^1_t)\mathds{1}_{(u^1_t=\lambda^1_t(x^1_t))}\pi^1_{t^+}(x^1_{t})\right)\times\left(\sum_{x_t^2}\sum_{u_t^2}\prob(X^2_{t+1}=x^2_{t+1}|x^2_t,u^2_t)\mathds{1}_{(u^2_t=\lambda^2_t(x^2_t))}\pi^2_{t^+}(x^2_{t})\right).
\end{align}
In equation $(a)$ in the display above, we drop $\lambda_t$ from $\prob(X_t  =x_{t}|z_{1:t},m^{1,2}_{1:t},\gamma_{1:t},\lambda_{1:t})$ since $\lambda_t$ is a function of the rest of the terms in the conditioning given the coordinator's strategy. Equation $(b)$ follows from the structure of the selection rule in \eqref{controlact1}. Equations $(c)$ and $(d)$ follow from the system dynamics (see \eqref{dyna}) and the conditional independence property in \eqref{factor2}. Further, we have
\begin{align}
\pi_{t+1}^i(x^i_{t+1}) = \sum_{x_t^i}\sum_{u_t^i}\prob(X^i_{t+1}=x^i_{t+1}|x^i_t,u^i_t)\mathds{1}_{(u^i_t=\lambda^i_t(x^i_t))}\pi^i_{t^+}(x^i_{t}), ~~ i = 1,2.
\end{align}
We denote the update rule described above with $\beta^i_t$, i.e.
\begin{align}
\pi_{t+1}^i = \beta_t^i(\pi_{t^+}^i,\lambda_t^i).
\end{align}





==> Erasure.tex <==
 Let's define variable $Z^{er}_t$ as:
\begin{equation}
  Z^{er}_t=\begin{cases}
    X^{1,2}_t, ~ w.p. ~~1-p_e & \text{if $M^{or}_t=1$}.\\
    \phi, ~ w.p. ~~p_e & \text{if $M^{or}_t=1$}.\\
    \phi, & \text{if $M^{or}_t=0$}.
  \end{cases}
\end{equation}
The information structure at each agent is given by 
\begin{equation}
    I^i_{t}=\{X^i_{1:t},U^i_{1:t-1},Z^{er}_{1:t-1},M^{1,2}_{1:t-1}\}
\end{equation}

==> MDP.tex <==
In this section we formulate the MDP problem to obtain optimal communication and control strategies.
We define variable $\tau_t$ as the last time instance when sharing happened between the agents 
\begin{equation}
  \tau_t=\begin{cases}
    max \{s \leq t-1,~~Z_s \neq \phi\}.\\
    1, \text{if~ $Z_s=\phi,~~ \forall s \leq t-1$}.
  \end{cases}
\end{equation}

and $\tau_{t^+}$ as the last time instance when sharing happened between the agents at time $t^+$.

\begin{equation}
  \tau_{t^+}=\begin{cases}
    \tau_t,~~ \text{if~ $Z_t=\phi$}.\\
    t, ~~~ \text{if ~$Z_t \neq \phi$}.
  \end{cases}
\end{equation}

The last time instance when sharing happened between agents at time $t+1$, is $\tau_{t+1}=\tau_{t^+}$ 

\begin{lemma}\label{lem:MDP}
Define $S_t=(X^{1,2}_{\tau_t},\gamma^{1,2}_{1+\tau_t:t-1},\lambda^{1,2}_{\tau_t:t-1})$ at time t and $S_{t^+}=(X^{1,2}_{\tau_{t^+}},\gamma^{1,2}_{1+\tau_{t^+}:t},\lambda^{1,2}_{\tau_{t^+}:t-1})$. Then:\\
 1) The process $\{S_t\}^T_{t=1}$ and $\{S_{t^+}\}^T_{t=1}$ are controlled Markov process with communication prescription $\gamma$ and control prescription $\lambda$, $t=1,2,....,T$,
 \begin{align}
     &\prob(S_{t^+}|S_{1:t}, \gamma_{1:t}, \lambda_{1:t-1})=\prob(S_{t^+}|S_{t}, \gamma_{t})\notag\\
     &\prob(S_{t+1}|S_{1:{t^+}},\gamma_{1:t}, \lambda_{1:t})=\prob(S_{t+1}|S_{{t^+}},\lambda_{t})
 \end{align}
     
 
2) The instantaneous conditional cost simplifies as follows
\begin{align}
    &\ee[\rho*\mathds{1}_{(M^{or}_t=1)}|S_{1:t}, \gamma_{1:t}, \lambda_{1:t-1}]=\ee[\rho*\mathds{1}_{(M^{or}_t=1)}|S_{t}, \gamma_{t}]\notag\\
    &\ee[c_t({X}_t,{U}_t)|S_{1:{t^+}},\gamma_{1:t}, \lambda_{1:t}]=\ee[c_t({X}_t,{U}_t)|S_{{t^+}},\lambda_{t}]   
\end{align}
\end{lemma}
see Appendix C for proof.

Using Lemma \ref{lem:MDP}, we can write a dynamic program for the simplified MDP problem. 
\begin{theorem}  For any realization $s_t$, $s_{t^+}$ of $S_t$ and $S_{t^+}$, we define Value function $~V_{T^+}(s_{T^+})$ after transmission at time $~T^+$:
\begin{align}
&V_{T^+}(s_{T^+}):=\notag\\
&\min_{\lambda_T}E\big[c_T(S_{T^+},\Lambda_T)|S_{T^+}=s_{T^+},\Lambda_T=\lambda_T \big]\notag\\
  &=c_T(s_{T^+},\lambda_T)
\end{align}
Value function $~V_{T}(s_{T})$ before transmission at time $T$:
\begin{align}
&V_{T}(s_{T}):=\notag\\
  &\min_{\gamma_T}E\big[\rho*\mathds{1}_{[m_T=1]}+V_{T^+}(S_{T^+})|S_{T}=s_{T},\Gamma_T=\gamma_T \big]\notag\\
  &=\rho*P[m_T=1|S_T,\gamma_T]\notag\\
  &+P[Z_T=\phi|S_T,\gamma_T]V_{T^+}(s_{T^+},\gamma_T)\notag\\
  &+\sum_{\tilde{x}_T^{1,2}}P(Z_T=x_T^{1,2}|S_T,\Gamma_T)V_{T^+}(\tilde{x}^1_T,\tilde{x}^2_T)]
\end{align}
and for $t=T-1,T-2,\ldots,1$, value function $V_{t^+}(s_{t^+})$ after transmission:
\begin{align}
&V_{t^+}(s_{t^+}):=\notag\\
  &\min_{\lambda_t}E\big[c_t(S_{t^+},\Lambda_t)+V_{t+1}(s_{t+1})|S_{t^+}=s_{t^+},\Lambda_t=\lambda_t \big]\notag\\
  &=c_t(s_{t^+},\lambda_t)+V_{t+1}(s_{t^+},\lambda_t)
\end{align}
Value function $V_{t}(s_{t})$ before transmission:
\begin{align}
&V_{t}(s_{t}):=\notag\\
    &\min_{\gamma_t}E\big[\rho*\mathds{1}_{[m_T=1]}+V_{t^+}(S_{t^+})|S_{t}=s_{t},\Gamma_t=\gamma_t \big]\notag\\
    &=\rho*P[m_t=1|S_t,\gamma_t]\notag\\
    &+P[Z_t=\phi|S_t,\gamma_t]V_{t^+}(s_{t^+},\gamma_t)\notag\\
    &+\sum_{\tilde{x}_t^{1,2}}P(Z_t=x_t^{1,2}|S_t,\Gamma_t)V_{t^+}(\tilde{x}^1_t,\tilde{x}^2_t)]
\end{align}

\end{theorem}

==> POMDP.tex <==
In this section we formulate the POMDP problem to obtain optimal control.\\
\begin{lemma}
Probability of $Z_t=\phi$ and $Z_t=\tilde{x_T^{1,2}}$ conditioned on belief state of agents and prescriptions for agents, $i=1,2$ is given by:
\begin{align}
    &P(Z_t=x_T^{1,2}|\pi_T^{1,2},\Gamma_T^{1,2}=\gamma_T^{1,2})\notag\\
    &=max(\gamma^1(x_T^{1}),\gamma^2(x_T^{2}))*\pi^1(x^1_T)\pi^2(x^2_T)\\
    &P(Z_t=\phi|\pi_T^{1,2},\Gamma_T^{1,2}=\gamma_T^{1,2})\notag\\
    &=\sum_{x_T^{1,2}}\mathbf{1}(\gamma^1(x_T^{1})=0),\mathbf{1}(\gamma^2(x_T^{2})=0)\pi^1(x^1_T)\pi^2(x^2_T)
\end{align}
\end{lemma}
\begin{proposition}[Nayyar et.al, Theorem 3] applied to model of Proposition 3) For any realization $\pi_t$, $\pi_{t^+}$ of $\Pi_t$ and $\Pi_{t^+}$, we define\\
 Value function $V_{T^+}(\pi_{T^+})$ after transmission at time $T^+$:
\begin{equation}
  \min_{\lambda_T}[\sum_{x_T^{1,2}}c_T(x_T^{1,2},\lambda^1(x_T^{1}),\lambda^2(x_T^{2}))\pi^1_{T^+}(x^1_T)\pi^2_{T^+}(x^2_T)]
\end{equation}
Value function $V_{T}(\pi_{T})$ before transmission at time $T$:
\begin{equation}
\begin{aligned}
\min_{\gamma_T}&[\rho*\sum_{x_T^{1,2}}max(\gamma^1(x_T^{1}),\gamma^2(x_T^{2}))\pi^1(x^1_T)\pi^2(x^2_T)\\ 
&+P(Z_t=\phi|\pi_T^{1,2},\Gamma_T^{1,2}) V_{T^+}(\eta( \Pi^{1,2}_{T},\Gamma^{1,2}_T))\\ &+\sum_{\tilde{x}_T^{1,2}}P(Z_t=x_T^{1,2}|\pi_T^{1,2},\Gamma_T^{1,2})V_{T^+}(\tilde{x}^1_T,\tilde{x}^2_T)]
\end{aligned}
\end{equation}
  
and for $t=T-1,T-2,...,1,$, value function $V_{t^+}(\pi_{t^+})$ after transmission:
\begin{align}
  \min_{\lambda_t}&[\sum_{x_t^{1,2}}c_T(x_t^{1,2},\lambda^1(x_t^{1}),\lambda^2(x_t^{2}))\pi^1_{t^+}(x^1_t)\pi^2_{t^+}(x^2_t)\notag\\
  &+V_{t+1}(\beta(\pi_{t^+},\lambda_t))]
\end{align}
Value function $V_{t}(\pi_{t})$ before transmission:
\begin{align}
\min_{\gamma_t}&[\rho*\sum_{x_t^{1,2}}max(\gamma^1(x_t^{1}),\gamma^2(x_t^{2}))\pi^1(x^1_t)\pi^2(x^2_t)\notag\\ 
&+P(Z_t=\phi|\pi_t^{1,2},\Gamma_t^{1,2}) V_{t^+}(\eta( \Pi^{1,2}_{t},\Gamma^{1,2}_t))\notag\\  &+\sum_{\tilde{x}_t^{1,2}}P(Z_t=x_t^{1,2}|\pi_t^{1,2},\Gamma_t^{1,2})V_{t^+}(\tilde{x}^1_t,\tilde{x}^2_t)]
\end{align}
\end{proposition}

